OT-VP: Optimal Transport-guided Visual Prompting for Test-Time Adaptation

Vision Transformers (ViTs) have demonstrated remarkable capabilities in learning representations, but their performance is compromised when applied to unseen domains. Previous methods either engage in prompt learning during the training phase or modify model parameters at test time through entropy minimization. The former often overlooks unlabeled target data, while the latter doesn't fully address domain shifts. In this work, our approach, Optimal Transport-guided Test-Time Visual Prompting (OT-VP), handles these problems by leveraging prompt learning at test time to align the target and source domains without accessing the training process or altering pre-trained model parameters. This method involves learning a universal visual prompt for the target domain by optimizing the Optimal Transport distance.OT-VP, with only four learned prompt tokens, exceeds state-of-the-art performance across three stylistic datasets-PACS, VLCS, OfficeHome, and one corrupted dataset ImageNet-C. Additionally, OT-VP operates efficiently, both in terms of memory and computation, and is adaptable for extension to online settings.

==> sec/fig/avg_across_num_prompts.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{img/avg_across_num_prompts.pdf}
    \caption{Effect of Prompt Length on OT-VP Performance. The performance of OT-VP exhibits only minor variations across different numbers of prompts, showing a robust improvement.}
    \label{fig:avg_across_num_prompts}
    \vspace{-0.5cm}
\end{figure}

==> sec/fig/boxplot_1src_pacs.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{img/boxplot_1src_pacs.pdf}
    \caption{PACS single-source violin plots}
    \label{fig:boxplot_1src_pacs}
\end{figure}

==> sec/fig/lambda_ablation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{img/lambda_ablation.pdf}
    \caption{Influence of hyperparameter $\lambda$ on ImageNet-C. Accuracy declines with smaller $\lambda$ values but stabilizes when $\lambda$ is large. These trends reveal the pivotal role of $\lambda$ in preventing cross-class transport and its impact on overfitting, particularly when using pseudo labels during prompt optimization.}
    \label{fig:lambda_ablation}
    \vspace{-0.5cm}
\end{figure}

==> sec/tab/algorithm.tex <==
\begin{algorithm}
\caption{OT-VP Algorithm}\label{alg:ot-vp_algo}
\textbf{Input:} Pre-trained feature extractor $\phi$ and classifier $h$,  visual prompts $\gamma$, source domain data $\mathcal{D}^s$, target unlabelled domain data $\mathcal{D}^t$, batch size $b$. \\

\textbf{Output:} Prediction for all target domain data.

\begin{algorithmic}
    \STATE \# Compute the source representations
    
\end{algorithmic}

\end{algorithm}

==> sec/tab/main_results.tex <==
\begin{table*}[ht]
    \centering
    \caption{Combined single-source and multi-source average results with enhancements}
    \label{tab:main_results}
    \begin{tabular}{lccc|ccc|c}
    \hline
    \multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{3}{c|}{\textbf{Single-Source}} & \multicolumn{3}{c|}{\textbf{Multi-Source}} & \multirow{2}{*}{\textbf{Average}} \\ \cline{2-7} 
                       & \textbf{PACS} & \textbf{VLCS} & \textbf{OfficeHome} & \textbf{PACS} & \textbf{VLCS} & \textbf{OfficeHome} &  \\ \hline
    ERM                & 61.2 & 63.8 & 66.5 & 87.1 & 78.5 & 73.6 & - \\
    DoPrompt           & -    & -    & -    & -    & -    & -    & - \\
    Tent-C             & 61.5 & 65.0 & 66.6 & 87.3 & 78.8 & 73.6 & - \\
    Tent-BN            & 67.1 & 58.5 & 67.6 & 87.0 & 73.5 & 74.6 & - \\
    T3A                & 69.1 & 68.3 & 67.8 & 87.6 & 80.0 & 74.7 & - \\
    OT-VP              & 68.8 & 65.2 & 66.7 & 87.3 & 80.2 & 74.3 & - \\
    OT-VP-L            & 70.8 & 68.4 & 67.8 & 87.8 & 80.9 & 75.1 & - \\ \hline
    \end{tabular}
\end{table*}
